Grounding Predicates through Actions

Symbols representing abstract states such as "dish in dishwasher" or "cup on table" allow robots to reason over long horizons by hiding details unnecessary for high-level planning. Current methods for learning to identify symbolic states in visual data require large amounts of labeled training data, but manually annotating such datasets is prohibitively expensive due to the combinatorial number of predicates in images. We propose a novel method for automatically labeling symbolic states in large-scale video activity datasets by exploiting known pre- and post-conditions of actions. This automatic labeling scheme only requires weak supervision in the form of an action label that describes which action is demonstrated in each video. We use our framework to train predicate classifiers to identify symbolic relationships between objects when prompted with object bounding boxes, and demonstrate that such predicate classifiers can match the performance of those trained with full supervision at a fraction of the labeling cost. We also apply our framework to an existing large-scale human activity dataset, and demonstrate the ability of these predicate classifiers trained on human data to enable closed-loop task planning in the real world.

==> tex/d-gridworld.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/4-gridworld.pdf}
    \caption{Gridworld environment. The goal of the agent is to obtain a $\obj{trophy}$ that is locked inside a $\obj{chest}$ locked inside another room. The sequence of actions shown here (1--14) is one of the solutions found by a PDDL solver to this long horizon planning problem.}
    \label{fig:3-gridworld}
\end{figure}

In this section, we provide details on the Gridworld environment. 

This synthetic 2D grid world environment is visualized in Fig~\ref{fig:3-gridworld}. In this environment, an agent needs to obtain a trophy from inside a chest. There are 8 objects: $\obj{agent}$, $\obj{trophy}$, $\obj{chest}$, $\obj{chest\_key}$, $\obj{door}$, $\obj{door\_key}$, $\obj{room\_a}$, and $\obj{room\_b}$. There are 6 predicates:
\begin{description}[labelindent=2pt,font=\normalfont]
    \item[-- $\prop{reachable a}$:] Whether $\obj{a}$ can be picked up by the agent.
    \item[-- $\prop{closed a}$:] Whether the door/chest $\obj{a}$ is closed.
    \item[-- $\prop{locked a}$:] Whether the door/chest $\obj{a}$ is locked.
    \item[-- $\prop{in a b}$:] Whether $\obj{a}$ is in $\obj{b}$.
    \item[-- $\prop{connects a b c}$:] Whether door $\obj{a}$ connects rooms $\obj{b}$, $\obj{c}$.
    \item[-- $\prop{matches a b}$:] Whether key $\obj{a}$ matches door/chest $\obj{b}$.
\end{description}
There are 8 actions to control the $\obj{agent}$:
\begin{description}[labelindent=2pt,font=\normalfont]
    \item[-- $\action{enter a b}$:] Enter room $\obj{a}$ through door $\obj{b}$.
    \item[-- $\action{goto a b}$:] Go to object $\obj{a}$ in room $\obj{b}$.
    \item[-- $\action{pick a b}$:] Pick up object $\obj{a}$ from object/room $\obj{b}$.
    \item[-- $\action{place a b}$:] Place object $\obj{a}$ inside object/room $\obj{b}$.
    \item[-- $\action{open a}$:] Open door/chest $\obj{a}$.
    \item[-- $\action{close a}$:] Close door/chest $\obj{a}$.
    \item[-- $\action{unlock a b}$:] Unlock door/chest $\obj{a}$ with key $\obj{b}$.
    \item[-- $\action{lock a b}$:] Lock door/chest $\obj{a}$ with key $\obj{b}$.
\end{description}

The actions are defined with complex pre- and post-conditions, making use of universal (\texttt{forall}), existential (\texttt{exists}), and conditional (\texttt{when}) quantifiers. See the \href{https://sites.google.com/stanford.edu/groundingpredicates}{project website} for the full PDDL specification.

To generate training data, we first sample a random symbolic state $s_0$, where each proposition in $s_0$ has a $5\%$ chance of being true. There are $172$ propositions in Gridworld, so on average, a randomly sampled state will have $8$ propositions. Then, given an action with its pre- and post-conditions $\hat{s}_{pre}$ and $\hat{s}_{post}$, we generate two symbolic states:
\begin{align}
    s_{pre}
        &= (s_0 \cup s_{pre}^+) - s_{pre}^- \\
    s_{post}
        &= (s_{pre} \cup s_{post}^+) - s_{post}^-
\end{align}

We then render $s_{pre}$ and $s_{post}$ to obtain $220 \times 220$ RGB images $\mathcal{I}_{pre}$ and $\mathcal{I}_{post}$, of which examples are shown in Fig.~\ref{fig:3-gridworld}.
